Building Robust Spoken Language Understanding by Cross Attention between Phoneme Sequence and ASR Hypothesis

Building Spoken Language Understanding (SLU) robust to Automatic Speech Recognition (ASR) errors is an essential issue for various voice-enabled virtual assistants. Considering that most ASR errors are caused by phonetic confusion between similar-sounding expressions, intuitively, leveraging the phoneme sequence of speech can complement ASR hypothesis and enhance the robustness of SLU. This paper proposes a novel model with Cross Attention for SLU (denoted as CASLU). The cross attention block is devised to catch the fine-grained interactions between phoneme and word embeddings in order to make the joint representations catch the phonetic and semantic features of input simultaneously and for overcoming the ASR errors in downstream natural language understanding (NLU) tasks. Extensive experiments are conducted on three datasets, showing the effectiveness and competitiveness of our approach. Additionally, We also validate the universality of CASLU and prove its complementarity when combining with other robust SLU techniques.

==> 02.related_work.tex <==
\section{Related Work}
Various approaches have been investigated in order to build SLU systems robust to ASR errors.
The most direct method is to detect and correct erroneous ASR hypotheses. Multi-feature and mutil-task are introduced to improve ASR error detection~\cite{DBLP:conf/icassp/TamLZW14,weng2020joint}.
%~\cite{DBLP:conf/interspeech/PellegriniT10,DBLP:conf/icassp/TamLZW14,weng2020joint}.
%Pellegrini and Trancoso~\cite{DBLP:conf/interspeech/PellegriniT10} include new features from different knowledge sources to improve ASR error detection, and Tam et al.~\cite{DBLP:conf/icassp/TamLZW14} propose a recurrent neural network language model for ASR error prediction.
%To correct ASR errors, techniques such as lexical co-occurrence statistics~\cite{DBLP:conf/naacl/SarmaP04}, machine translation~\cite{DBLP:conf/interspeech/DHaroB16,mani2020towards}, and noisy channel model~\cite{DBLP:journals/corr/abs-1802-02607} have also been explored.
%Notably, Weng et al.~\cite{weng2020joint} jointly train a contextual ASR error correction system along with NLU to improve the performance of both tasks simultaneously.
%Instead of correcting ASR errors, 
Another line of research focuses on leveraging information on ASR outputs and incorporates them within downstream NLU model.
Lattice~\cite{ladhak2016latticernn,huangchen2020learning}
%~\cite{ladhak2016latticernn,huang2019adapting,huangchen2020learning} 
and word confusion networks~\cite{tur2013semantic,shivakumar2019spoken}
%~\cite{tur2013semantic,shivakumar2019confusion2vec,shivakumar2019spoken}
are employed to model the token-level confidence of ASR outputs.
%~\cite{tur2002improving,hakkani2006beyond,tur2013semantic,shivakumar2019confusion2vec,shivakumar2019spoken} are employed to model the token-level confidence of ASR outputs.
To handle the ASR uncertainty at utterance level, n-best hypotheses are also commonly used through implicit and explicit weighting~\cite{li2020multi,li2020improving,liu2021asr} or reranking~\cite{ogawa2018rescoring,ogawa2019improved}.
%~\cite{kumar2017use,ogawa2018rescoring,ogawa2019improved}.
Despite the success of these methods, using only texts generated by ASR module unavoidably loses fine-grained speech information, e.g. prosody and intonation.
%, and prior work has proved that they are helpful for improving the robustness of SLU models.For instance, 
Therefore, end-to-end (E2E) SLU systems take audio signals as input to perform the downstream task directly~\cite{haghani2018audio,serdyuk2018towards,lugosch2019speech,tomashenko2019investigating}.
%, bypassing the error-prone generation from intermediate ASR system~\cite{haghani2018audio,serdyuk2018towards,lugosch2019speech,tomashenko2019investigating}.
%Multi-modal pretraining for speech and text has also attracted much attention~\cite{DBLP:conf/naacl/ChungZZ21,9414619,DBLP:journals/corr/abs-2102-06283}, as large-scale unannotated data in both modalities can be exploited and the pretrained model can produce richer representations for downstream task fine-tuning.
In addition to audio features, which may vary greatly across people and could be distorted by different noise sources, phoneme is considered a cleaner form of sound information.
It has been used, complementary to raw text, to enhance the robustness of NLU~\cite{yenigalla2018speech, fang2020using, sundararaman2021phoneme,9414558}. 
%For example, Yenigalla et al. \cite{yenigalla2018speech} utilize phoneme embeddings to facilitate speech emotion recognition. Fang et al. \cite{fang2020using} explore word2vec to learn phoneme embeddings, aiming to capture pronunciation similarities of phonemes. Sundararaman et al. \cite{sundararaman2021phoneme} propose a BERT-style language model to learn phonetic-aware representations, which are robust to ASR errors. Kim et al.~\cite{9414558} feed phoneme posterior and subword-level text into a BERT-based model, and pretrain a contextualized cross-modal alignment via multiple objectives.
Our work also falls in this area of using phoneme-enhanced methods, but we aim to explicitly model the interactions between ASR phonemes and hypotheses.
